Bayesian Incentive-Compatible Bandit Exploration

Individual decision-makers consume information revealed by the previous decision makers, and produce information that may help in future decisions. This phenomenon is common in a wide range of scenarios in the Internet economy, as well as in other domains such as medical decisions. Each decision-maker would individually prefer to "exploit": select an action with the highest expected reward given her current information. At the same time, each decision-maker would prefer previous decision-makers to "explore", producing information about the rewards of various actions. A social planner, by means of carefully designed information disclosure, can incentivize the agents to balance the exploration and exploitation so as to maximize social welfare. We formulate this problem as a multi-armed bandit problem (and various generalizations thereof) under incentive-compatibility constraints induced by the agents' Bayesian priors. We design an incentive-compatible bandit algorithm for the social planner whose regret is asymptotically optimal among all bandit algorithms (incentive-compatible or not). Further, we provide a black-box reduction from an arbitrary multi-arm bandit algorithm to an incentive-compatible one, with only a constant multiplicative increase in regret. This reduction works for very general bandit setting that incorporate contexts and arbitrary auxiliary feedback.

==> sec-results.tex <==
\section{Our technical results in more detail (DEPRECATED!)}

\ascomment{This is basically "our contributions" from the old intro, minus the material already in the new intro or the prelims. But I would probably need to do a more thorough pass.}

\xhdr{BIC bandit exploration}
We provide a BIC algorithm whose regret is essentially optimal among all MAB algorithms with a constant number of actions, both in the ``instance-dependent" sense and in the worst case over all MAB instances. We achieve regret
\begin{align}\label{eq:intro-MAB-regret}
    c_\mP \log(T) + c_0\cdot\min(\tfrac{1}{\Delta} \log T, \sqrt{T\log T}),
\end{align}
where $T$ is the time horizon, $\Delta$ is the gap, $c_0$ is an absolute constant, and $c_\mP$ is a constant that depends only on the common prior $\mP$. A well-known lower bound states that one cannot achieve regret better than
     $O(\min(\tfrac{1}{\Delta} \log T, \sqrt{T}))$.%
\footnote{More precisely: any MAB algorithm has regret at least
    $\Omega(\min(\tfrac{1}{\Delta} \log T, \sqrt{T}))$
in the worst case over all MAB instances with two actions, time horizon $T$ and gap $\Delta$ \cite{Lai-Robbins-85,bandits-exp3}.}

\ascomment{need to define the gap somewhere.}

\OMIT{We also consider \emph{Bayesian regret} --- regret in expectation over the prior --- and improve the $ c_\mP\, \sqrt{T\log T}$ regret bound (which trivially follows from \eqref{eq:intro-MAB-regret}) to regret
    $ c_\mP\,\log(T) + C_0\,\sqrt{T\log T}$,
where $C_0$ is an absolute constant.}

Further, our algorithm is \emph{detail-free}, in the sense that it requires very little knowledge of the common prior $\mP$. This is desirable because in practice it may be complicated or impossible to elicit the  prior exactly. The prior is taken into account through the ranking $\rho_\mP$ of the actions in terms of their prior mean rewards and two numbers $k_{\mP}^*$ and $L_\mP$ which are related to the strength of the agents' initial beliefs in favor of some arm. The algorithm is parameterized by the ranking $\rho_\mP$ and two numbers $k^*$, $L$ (number of samples collected in the initial stage of the algorithm and phase length in the initial stage of the algorithm) such that the algorithm is BIC as long as $k^*>k_{\mP}^*$ and $L\geq L_\mP$, and the prior-dependent constant is $c_\mP = O(L\cdot k^*)$. Moreover, computing these two constants $k_{\mP}^*$ and $L_{\mP}$ requires only minimal knowledge of the prior distribution of each mean (only the expected value of each prior and the value of the cumulative density function at two points). This result has some surprising practical consequences:

\begin{itemize}
\item Agents can have different priors $\mP$ as long as they are ``compatible" with the planner's prior: agree on the ranking $\rho_\mP$ and satisfy $k_{\mP}^*<k^*$ and $L_\mP\leq L$.
\item An agent does not need to know her own prior. She would trust the planner's algorithm recommendation as long as she believes that their priors are ``compatible", in the above sense.
\end{itemize}

%\subsection{Our contributions: a general ``black-box" reduction}
%\label{sec:contributions-BB}

\xhdr{A general ``black-box" reduction.}
We provide a ``black-box" reduction from MAB algorithms to BIC algorithms. Given an arbitrary MAB algorithm $\ALG$, we provide a BIC algorithm $\ALGIC$ that interleaves exploitation and calls to $\ALG$. We focus on \emph{Bayesian regret} of $\ALGIC$ in $T$ rounds --- regret in expectation over the prior $\mP$, denoted $R_\mP(\ALGIC;T)$.
Bayesian regret of $\ALGIC$ increases by at most a constant multiplicative factor $c_\mP$ that only depends on the prior $\mP$:
\begin{align*}
   \textstyle{ R_\mP(\ALGIC; T) \leq c_\mP \cdot R_\mP(\ALG;\, T).}
\end{align*}

Further, our reduction incurs very little loss in terms of the average reward. Specifically, let $V_\mP(\ALG;[\tau_1,\tau_2])$ be the average expected reward per agent among the agents in
the time interval $[\tau_1,\tau_2]$, if they follow algorithm $\ALG$ when the prior is $\mP$. Then
\begin{align*}
  \textstyle{  V_\mP(\ALGIC; [c_\mP+1,T+c_\mP]) \geq  V_\mP(\ALG;\, [1,T/L_\mP]),}
\end{align*}
where $c_\mP$ and $L_\mP$ are two constants that depend only on the prior $\mP$.
In words, if we ignore the first $c_\mP$ agents in the execution of $\ALGIC$, the average expected reward per agent for the next $T$ agents is at least that of the first $T/L_\mP$ agents in the original algorithm $\ALG$.

While our primary motivation comes from maximizing the social welfare, our reduction is much more general, and can handle {\em any} MAB algorithm. In particular, as discussed in the Introduction, the MAB algorithm may learn an action that is optimal based on criteria other than the agents' utility.

\OMIT{Our ``black-box" reduction is based on a variant of the same technique as the previous algorithm. Conceptually, it demonstrates that our technique is not tied to a specific approach to exploration.}


%\subsection{Our contributions: the ``black-box" reduction in a general setting}
%\label{sec:contributions-general}

\xhdr{The ``black-box" reduction in a general setting.}
We also extend the ``black-box" reduction result to a much more general setting where each agent comes with a signal (\emph{context}) which can include demographics, tastes, preferences and other agent-specific information. The context, observable by both the agent and the algorithm, impacts the rewards received by this agent, as well as the agent's beliefs about these rewards. Formally, in each round one has context $x$ and expected reward $r_a$ for each action $a$ in the action set $A$, so that the tuple $(x; r_a: a\in A)$ is drawn IID from some distribution $\mD$, called \emph{contextual MAB instance}. This distribution is not known neither to the agents nor to the algorithm. However, both the agents and the algorithm share a publicly known Bayesian prior $\mP$ on the contextual MAB instance. When the context $x$ is revealed, an agent can update her Bayesian posterior on the rewards. In particular, this allows agents to have different beliefs about their rewards.

Absent the BIC requirement, the machine learning problem reduces to \emph{contextual bandits} with IID rewards/contexts \citep{Langford-nips07}. An algorithm's performance is measured relative to the best \emph{policy} --- mapping from contexts to actions --- in a given class $\Pi$ of feasible policies. One defines \emph{contextual regret}: informally, the extent to which the algorithm ``regrets" not knowing the best policy in advance, quantified as a loss in expected reward. One is primarily interested in the asymptotic dependence of contextual regret on the time horizon $T$ and the number of policies $|\Pi|$. The optimal dependence is, resp., $\tilde{O}(\sqrt{T})$ and $O(\sqrt{\log |\Pi|})$ \citep{policy_elim}.

Contextual bandits is a very flexible setting, as the policy class $\Pi$ can encode problem-specific structure and/or available heuristics for supervised learning. Algorithms are typically stated for an arbitrary $\Pi$, which is then represented via an oracle that implements supervised learning over $\Pi$. Even a single such algorithm in fact represents a collection of algorithms, one for each oracle. Ideally, one would like to provide a BIC implementation for all of these algorithms. This makes a general reduction result particularly desirable.

\vspace{2mm}
{\em Our results.}
We provide a reduction from an arbitrary contextual bandit algorithm $\ALG$ to a BIC algorithm $\ALGIC$ for our setting. We focus on the \emph{Bayesian contextual regret} of $\ALGIC$: contextual regret in expectation over the prior $\mP$; denote it $R_\mP(\ALGIC; T, |\Pi|)$. We prove that the Bayesian contextual regret of $\ALGIC$ increases compared to that of $\ALG$ by at most a constant multiplicative factor $c_\mP$ that only depends on $\mP$:
\begin{align*}
    \textstyle{R_\mP(\ALGIC; T,|\Pi|) \leq c_\mP \cdot R_\mP(\ALG;\, T, |\Pi|).}
\end{align*}

Further, apart from (or even instead of) optimizing social welfare, an algorithm may be learning something over time. The most natural object to learn in a contextual MAB setting is the best policy:   a policy $\pi\in\Pi$ with the largest expected reward for a given contextual MAB instance. To model this, we can assume that $\ALG$ outputs a predicted best policy $\pi_t\in \Pi$ after each round $t$. More generally, we assume that $\ALG$ outputs a \emph{prediction} $\phi_t\in \Phi$ after each round $t$, where $\Phi$ is some fixed set of possible predictions.

Our BIC algorithm $\ALGIC$ learns as fast as $\ALG$, up to a constant factor. Formally, $\ALGIC$ outputs a prediction $\phi^*_t\in \Phi$ after each round $t$, with the following guarantee: for every fixed contextual MAB instance and each round $t$, the prediction $\phi^*_t$ has the same distribution as $\phi_{\flr{t/c_\mP}}$. (Here $c_\mP$ is a constant that depends only on the prior $\mP$.) For example, if $\ALG$ gives an asymptotically optimal error rate $O(t^{-1/2})$ for learning the best policy, then so does $\ALGIC$, up to a prior-dependent multiplicative factor.

\vspace{2mm}
{\em Extensions.} In practice, agents' choices may reveal more information than respective rewards. For example, an agent's review of a given restaurant may contain not only the agents' evaluation of her experience in this restaurant (i.e., her reward), but also her opinions about the cuisine to which this restaurant belongs. The latter represents partial information about the rewards of some other actions.

We extend the above results to a machine learning setting with arbitrary feedback structure: in each round, the outcome of choosing a given action $a\in A$ includes not only the agent's reward $r_a$ for this action but also arbitrary additional feedback $f_a$ observed by the algorithm. The IID assumption extends to the feedback: the tuple
    $(x;\, r_a, f_a: a\in A)$
is drawn IID from some latent distribution $\mD$. The contextual bandit algorithm $\ALG$ can incorporate this additional feedback in an arbitrary way, and our BIC algorithm $\ALGIC$ matches $\ALG$ up to a constant factor, in the same sense as above.



